Approximation of integral operators using convolution-product expansions

We consider a class of linear integral operators with impulse responses varying regularly in time or space. These operators appear in a large number of applications ranging from signal/image processing to biology. Evaluating their action on functions is a computation-ally intensive problem necessary for many practical problems. We analyze a technique called convolution-product expansion: the operator is locally approximated by a convolution, allowing to design fast numerical algorithms based on the fast Fourier transform. We design various types of expansions, provide their explicit rates of approximation and their complexity depending on the time varying impulse response smoothness. This analysis suggests novel wavelet based implementations of the method with numerous assets such as optimal approximation rates, low complexity and storage requirements as well as adaptivity to the kernels regularity. The proposed methods are an alternative to more standard procedures such as panel clustering, cross approximations, wavelet expansions or hierarchical matrices.

==> body/SVD.tex <==
\section{Adaptive decompositions}

In \cite{flicker2005anisoplanatic}, the authors proposed to use a singular value decomposition (SVD) of the TVIR in order to construct the functions $h_k$ and $w_k$. 
In this section we first detail this idea and then analyze it from an approximation theoretic point of view.
Let $J:L^2(\Omega)\to L^2(\Omega)$ denote the linear integral operator with kernel $T\in \mathcal{T}^s$. 
First notice that $J$ is a Hilbert-Schmidt operator since $\|J\|_{HS}=\|H\|_{HS}$.
By lemma \ref{lem:schmidt} and since Hilbert-Schmidt operators are compact, $J$ can be decomposed as
\begin{equation}
  J = \sum_{k\geq 1} \sigma_k \cdot e_k \otimes f_k,
\end{equation}
leading to
\begin{equation}\label{eq:decomposition_svd_T} 
 T(x,y)= \sum_{k=1}^{+\infty} \sigma_k f_k(x) e_k(y).
\end{equation}

\begin{theorem}
For a given $m$, the set of functions $(h_k)_{1\leq k\leq m }$ and $(w_k)_{1\leq k\leq m }$ that minimizes $\|H_m - H\|_{HS}$ is given by:
\begin{equation} 
h_k = \sigma_k f_k \quad \textrm{and} \quad w_k = e_k.
\end{equation}
Moreover, if $T(x,\cdot) \in W^{s,2}(\Omega)$ for all $x\in \Omega$, we get:
\begin{equation} \label{eq:svd_rate}
\|H_m - H\|_{HS} = O\left( m^{-s} \right).
\end{equation}
In addition, for all $\epsilon > 0$, there exists an operator $H$ with TVIR in $\mathcal{T}^s$ such that:
 \begin{equation}\label{eq:svd_lowerbound}
  \|H_m - H\|_{HS} \geq m^{-(s+\epsilon)}.
 \end{equation}
\end{theorem}
\begin{proof}
 The proof of \eqref{eq:svd_rate} is standard. 
 We wish to solve:
 \begin{equation}
  \min_{T_m\in L^2(\Omega\times \Omega),\  \mathrm{rank}(T_m)=m} \|T_m-T\|_{L^2(\Omega\times \Omega)}.
 \end{equation}

 First notice that the set of functions $(g_{i,j})$ defined by $g_{i,j}(x,y)=f_i(x)e_j(y)$ is an orthonormal basis for $L^2(\Omega\times \Omega)$.
 Therefore $T$ and $T_m$ can be decomposed uniquely as
 \begin{equation}
  T(x,y) = \sum_{i,j} \sigma_{i,j} g_{i,j}, 
 \end{equation}
  \begin{equation}
  T_m(x,y) = \sum_{i,j} \tilde\sigma_{i,j} g_{i,j}.
 \end{equation}

By \eqref{eq:decomposition_svd_T}, we have $\sigma_{i,j}=0, \ \forall i\neq j$ and $\sigma_{i,i}=\sigma_i$. By Parseval identity:
 \begin{align}
  \|T_m-T\|_{L^2(\Omega\times \Omega)} &= \sum_{i,j} (\sigma_{i,j} - \tilde \sigma_{i,j})^2.
 \end{align}
The choice that minimizes this energy is $\tilde \sigma_{i,j} = 0, \ i\neq j$, $\tilde \sigma_{i,i} = \sigma_i, \ i\in \{1,\hdots, m\}$ and $\tilde \sigma_{i,i} = \sigma_i, \ i>m$.
This corresponds to defining $T_m$ as:
 \begin{equation} \label{eq:svd_form}
 T_m(x,y)= \sum_{k=1}^{m} \sigma_k f_k(x) e_k(y). 
 \end{equation}
 Since $T_m$ is the best rank $m$ approximation of $T$, it is necessarily better than bound \eqref{eq:Fourier_rate}, yielding \eqref{eq:svd_rate}.
  
 
 In order to prove, \eqref{eq:svd_lowerbound}, we construct a ``worst case'' TVIR $T$ defined as follows:
 \begin{equation}\label{eq:svd_construction}
  T(x,y) = \sum_{|k| \leq N} \sigma_k f_k(x) \bar f_k(y),
 \end{equation}
 where $f_k(x) = \exp(-2i\pi k x)$ is the $k$-th Fourier atom, $\sigma_0=0$ and $\sigma_k = \sigma_{-k} = \frac{1}{|k|^{s+1/2+\epsilon/2}}$ for $|k|\geq 1$.
 First, we prove that $T\in \mathcal{T}^s$. Notice that the Fourier series of $T(x,\cdot)$ is given by $\sigma_k f_k(x)$ which is bounded by $\sigma_k$. 
 By lemma \ref{lem:Characterization_Fourier_Sobolev}, $T(x,\cdot)$ therefore belongs to $W^{s,2}$ for all $x\in \Omega$. 
 By construction, the spectrum of $T$ is $(\sigma_k)_{k\in \N}$, therefore for any rank $m$ approximation of $T$, we get:
 \begin{align}
  \|T-T_m\|_{HS}^2 & \geq \sum_{|k|\geq m+1} \frac{1}{|k|^{2s+1+\epsilon}} \\
  & \geq  \int_{m}^\infty \frac{2}{t^{2s+1+\epsilon}} \,dt \\
  & = \frac{1}{2s+\epsilon} \frac{2}{m^{2s+\epsilon}}.
  \end{align}
\end{proof}

Even if the SVD gives an optimal decomposition, there is no guarantee that functions $e_k$ are supported on an interval of small size. 
As an example, it suffices to consider the ``worst case'' TVIR given in equation \eqref{eq:svd_construction}.
Therefore functions $w_k$ are generically supported on intervals of size $p = n$. This yields the following proposition.

\begin{corollary}
Let $\epsilon>0$  and set $m = \lceil C \epsilon^{-s}\rceil$. Then $H_m$ satisfies $\| H - H_m \|_{HS} \leq \epsilon$ and the matrix-vector with $H_m$ can be evaluated with no more than $O(\epsilon^{-1/s} n \log n)$ operations.
\end{corollary}



==> body/numerical.tex <==
\section{Numerical experiments}\label{sec:numerical}
